Kanana: Compute-efficient Bilingual Language Models

We introduce Kanana, a series of bilingual language models that demonstrate exceeding performance in Korean and competitive performance in English. The computational cost of Kanana is significantly lower than that of state-of-the-art models of similar size. The report details the techniques employed during pre-training to achieve compute-efficient yet competitive models, including high quality data filtering, staged pre-training, depth up-scaling, and pruning and distillation. Furthermore, the report outlines the methodologies utilized during the post-training of the Kanana models, encompassing supervised fine-tuning and preference optimization, aimed at enhancing their capability for seamless interaction with users. Lastly, the report elaborates on plausible approaches used for language model adaptation to specific scenarios, such as embedding, retrieval augmented generation, and function calling. The Kanana model series spans from 2.1B to 32.5B parameters with 2.1B models (base, instruct, embedding) publicly released to promote research on Korean language models.

==> adaptation/function_calling.tex <==
\subsection{Function Calling}
Function calling is the ability to reliably connect LLMs to external tools to enable effective tool usage and interaction with external APIs. We constructed training data based on the Korean language. As a result, we achieved a model with outstanding performance in Korean.\par

The evaluation utilized FunctionChat-Bench \citep{lee2024functionchat}, which is constructed with Korean evaluation data. Single-call evaluates how accurately the model can select and call the necessary function among several options. Dialogue evaluates how accurately the model responds in multi-turn situations.
\begin{table}[hbt!]
\centering
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{lrr}
\toprule
Models & \begin{tabular}[c]{@{}l@{}}\textbf{Single-call} \end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Dialogue}\end{tabular}  \\
\midrule
gpt-4o-2024-05-13     & 0.93    & \textbf{0.95}    \\
gpt-4-0125-prevew & \textbf{0.94}   & 0.94  \\
gpt-3.5-turbo-0125 & 0.92 & 0.89 \\
\midrule
Llama3-cpt-8b-instruct &  &  \\
\hspace{1em}+ single  & 0.89    & 0.74    \\
\hspace{1em}+ multi   & \textbf{0.94}     & 0.76    \\
\hspace{1em}+ multi + sgd  & 0.82  & 0.84    \\
Kanana Essence 8B Instruct &  &  \\
\hspace{1em}+ multi + sgd & 0.81   & 0.83  \\
\hspace{1em}+ multi + sgd + synthetic\_single & 0.88  & \textbf{0.89} \\
\bottomrule
\end{tabular}
}
\caption{Accuracy of FunctionChat-Bench}\label{tab-fc-overall}
\end{table}
\par
The experiment utilizes two models. One is a model that performs continual pre-training on 500 billion Korean and English datasets using the LLama3-8B\footnote{\url{https://huggingface.co/meta-llama/Meta-Llama-3-8B}} model, followed by instruct tuning. This model is referred to as llama3-cpt-8b-instruct. Another one is an 8B-sized model trained from-scratch and then instruct tuned. We refer to this model as Kanana Essence 8B Instruct. This model has high performance in the Korean language because it has extensively learned from Korean data. Our GPT results utilized zero-shot. Our model achieved more than 90\% performance compared to the GPT model in both Single-call and Dialogue.


\subsubsection{Data}
The datasets are comprised of public datasets \citep{rastogi2020towards, liu2024apigen} and private dataset (synthetic\_single). The internally developed dataset is called the private dataset.  Figure \ref{fig:fc_dataset} outlines the process for generating training data.\par
We used different combinations of datasets for each training stage. Specifically, stage-1 primarily consists of English data, while stage-2 is composed solely of Korean data. We uniformly divided the final constructed dataset into a 9:1 ratio to form the training and validation sets.
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.37]{figures/function_calling/fc_dataset.pdf}
    \caption{Construction process of function calling dataset}
    \label{fig:fc_dataset}
\end{figure}

\subsubsection{Multi-staged Training}
First, post-training with function call training data is performed to strengthen the understanding of contextual meaning and domain terminology\citep{whang2019effective}. This is defined as stage-1. In particular, at this stage, English data is incorporated to address the issue of insufficient data.\par

Stage-2 is defined as the step where supervised fine-tuning is performed to execute actual function calling. In this stage, only Korean data is used. Figure \ref{fig:fc_multi_stage} illustrates the overall training process.\par

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/function_calling/fc_multi_stage.pdf}
    \caption{Multi-stage training process}
    \label{fig:fc_multi_stage}
\end{figure}

\textbf{Stage-1} The base model has never been exposed to the function calling dataset before, so it needs to adapt to this dataset. In addition, chat template associated with function calls can use various special tokens (e.g., \big|function\big|). If this special token is one that has never been encountered in the base model or pre-trained model, then it cannot adequately learn the information about the token through the supervised fine-tune stage alone. This is because the fine-tune dataset often contains only a small amount of data. This deficiency can be overcome through the post-training process. \par

There are various examples of functions in different forms and their call results included in the publicly available English datasets.  By utilizing this during the post-training phase, one can effectively use rich information while minimizing the impact on Korean language performance. We use the NTP-loss and apply masking to special tokens in the input labels. Masking is used to exclude certain tokens from loss calculation.\par

\textbf{Stage-2} Once post-training is completed, further training is conducted. In stage-1, special tokens were masked. In this stage, only the output necessary for actual function calling is produced by masking user input and function call results. For user queries, the function calling model outputs the function to be called along with its parameters, and it is trained to generate an appropriate natural language response based on the function call results.\par
Through this, one can learn the ability to distinguish between cases where a function call is necessary and those where it is not. Additionally, it develops the ability to fill in missing arguments for function calls through re-quring. This stage is identical to stage 1, except for the difference in the region of masking on the input data.\par




==> adaptation/rag.tex <==
\subsection{Retrieval-Augmented Generation}
In this section, we describe a process of developing reliable RAG models with enhanced fluency, coherence, and factual accuracy from Kanana LLMs and introduce internal Korean RAG benchmark developed to more accurately measure the factual consistency.

% The evaluation of diverse models of korean RAG scenarios is presented in \autoref{fig:rag-main-performance}.
% After our training process, Kanana Essence 9.8B RAG achieved helpfulness while maintaining 91.4\% of GPT-4o's grounding performance. So we comfirmed that Kanana model can sufficiently achieve grounding performance against oracle model.

\begin{figure}[h]
    \small
    \centering
    \includegraphics[width=0.6\textwidth]{figures/rag/rag-main-performance-iter4.pdf}
    \caption{Performance Comparison of Various Models Based on averaged helpfulness and grounding in RAG-General-Bench.}
    % \caption{Performance Overview}
    \label{fig:rag-main-performance}
\end{figure}
Retrieval-Augmented Generation (RAG) methods \citep{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp} enable large language models to access the latest external or proprietary information without altering model parameters \citep{liu2024chatqasurpassinggpt4conversational}.
% Retrieval-Augmented Generation (RAG) is a hybrid generation model that combines Large Language Models (LLMs) with access to non-parametric memory \citep{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp}.
With access to reliable data sources, such as search results, data bases, and tool call, RAG greatly reduces the hallucination of LLMs \citep{Shuster2021RetrievalAR}.
% In other words, it enhances reliability and contextual accuracy by ensuring that generated responses are conditioned on the given information from credible sources, such as search, database, and tool call.
% To ensure advantages of RAG, additional training process is required to enhance factuality \citep{lin2024flamefactualityawarealignmentlarge}.
However, in order to endow RAG ability, models require further training using appropriate RAG data \citep{lin2024flamefactualityawarealignmentlarge}.
% Additionally, robust evaluation methods are crucial to accurately measure factual consistency for model ablation.

\begin{figure}[h]
\centering
\resizebox{0.9\textwidth}{!}{%
    \includegraphics[width=\textwidth]{figures/rag/data-generation-pipeline.pdf}
}
\caption{QA Generation Pipelines}
\label{fig:rag-data-generation-pipeline}
\end{figure}

% To encourage responses that leverage contextual information, 
To construct RAG dataset, we synthetically generate question-answer pairs  using high-quality bilingual documents as seed documents, following the pipeline in \autoref{fig:rag-data-generation-pipeline}.
% We build dataset around specialized knowledge to ensure that model relies on contextual information rather than its intrinsic knowledge.
% We construct a dataset that requires specialized knowledge to respond, to 
% After generation of large amount of QA pair, we filter low-grounded responses with LLM-Judge and then execute response refinement with reflection, ensuring that only high-grounded responses remained.
From the synthetically generated pairs, we filter out instances with low grounding scores and use LLM-judge to reflect and refine the low grounding instances.
At this point, we have obtained dataset for SFT, which we call SynQA-SFT. 
Along with SynQA-SFT, we augment StructLM \citep{zhuang2024structlmbuildinggeneralistmodels}, FollowRAG \citep{dong2024generalinstructionfollowingalignmentretrievalaugmented}, and SFT dataset from Section \ref{subsec:post-training-data} to train the instruction model to adapt to the RAG scenarios.
% while maintaining its instruction following capabilities.
Then, we augment low grounding responses to high grounding instances in SynQA-SFT to construct preference dataset for DPO.
Because the SFT and DPO process decays instruction following capability, we merge the DPO model with the instruction model to preserve both abilities.
% To execute the pipline cost-effectively, we utilized strong model for generation and LLM-Judge locally served.
Our comprehensive training process demonstrates improvements in grounding performance while maintaining the instruction following scores, as shown in \autoref{tab:rag-performance-comparison}.

% During training phase, we focus on improving grounding capability.
% In SFT phase, we utilize a mixture of StructLM \citep{zhuang2024structlmbuildinggeneralistmodels}, FollowRAG \citep{dong2024generalinstructionfollowingalignmentretrievalaugmented} and synthetic QA dataset for training to adapting diverse context format and instructions in RAG scenarios. Additionally, we replay SFT dataset from Section \ref{subsec:post-training-data} to maintain helpfulness and instruction-following capabilities.
% During DPO phase, we inject preference for better grounding responses by augmenting rejected responses.
% Our comprehensive training process demonstrates improvements in grounding performance as shown in \autoref{tab:rag-performance-comparison}.
    
% However, it also declines helpfulenss compared to base model.  
% To address this issue, we apply weight averaging at the end of process. To enhance overall performance, grounding-focused model was merged with helpfulness-focused model.
% When merging models with different concepts, task transfer could be possible in addition to the ensemble effect \citep{kim2024prometheus2opensource}.
% Through this approach, we can get also higher score of helpfulness compared to base model.

\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|cc|c|c}
    \toprule
    \textbf{Models} & \multicolumn{1}{c|}{\textbf{FACTs}} & \multicolumn{2}{c|}{\textbf{RAG-General-Bench}} & \multicolumn{1}{c|}{\textbf{ContextualBench}} & \multicolumn{1}{c}{\textbf{IFEval}} \\
    & \small{grounding} & \small{grounding} & \small{helpfulness} & \small{em} &  \\
    \midrule
    Kanana Essence 9.8B & 40.66 & 32.63 & 55.86 & 20.22 & \textbf{79.93}\\
    \midrule
    % Phase1 (SFT)& 62.40& 59.29& 51.60& 48.08& 72.99\\
    % Phase2 (DPO)& \textbf{63.09}& \textbf{65.33}& 52.67& \textbf{48.76}& 75.00\\
    % Phase3 (Merge)& 53.09 & 57.38& \textbf{57.32}& 48.31& 78.44\\
    + SFT & 62.40& 59.29& 51.60& 48.08& 72.99\\
    + DPO & \textbf{63.09}& \textbf{65.33}& 52.67& \textbf{48.76}& 75.00\\
    + Merge (Kanana Essence 9.8B RAG) & 53.09 & 57.38& \textbf{57.32}& 48.31& 78.44\\
    \bottomrule
    \end{tabular}
}
    \caption{Performance change of each phase of recipe. Grounding score is average of RAGAS \citep{es2023ragasautomatedevaluationretrieval} Faithfulness and rubric based LLM-judge. Helpfulness score is average of RAGAS Answer Relevancy and rubric based LLM-judge.}
    \label{tab:rag-performance-comparison}
\end{table}
    

% \begin{wrapfigure}[14]{r}{0.45\textwidth}
%     \centering
%     \resizebox{0.44\textwidth}{!}{%
%         \includegraphics{figures/rag/eval-ko-data-portion.pdf}
%     }
%     \caption{Task distribution of RAG-General-Bench, which was developed by Kanana team.}
%     \label{rag-ko-eval-data}
% \end{wrapfigure}

For completeness of the evaluation, we collect and assess our model on diverse RAG scenario benchmarks of ContextualBench \citep{nguyen2024sfrragcontextuallyfaithfulllms}, FACTs \citep{jacovi2025factsgroundingleaderboardbenchmarking}, and IFEval \citep{zhou2023instructionfollowingevaluationlargelanguage}.
% ContextualBench \citep{nguyen2024sfrragcontextuallyfaithfulllms} is set of multi-hop QA testset that golden answers are highly concise rather than chat-style. 
% we utilized it for measure conciseness of response and intuitive evaluation method based on exact match.
% FACTs \citep{jacovi2025factsgroundingleaderboardbenchmarking} is consist of diverse task given context like Reasoning, QA, Summarization, Rewriting and Extraction. 
% We filtered within char-level length 20k since our base model was trained with token length limit of 8k. This dataset is not labeled golden answer, so we only measure grounding score with it.
% IFEval \citep{zhou2023instructionfollowingevaluationlargelanguage} measures the maintenance of instruction following performance. 
% While utilizing english public benchmarks, we developed internal RAG benchmark named RAG-General-Bench to address insufficient of korean evaluation set.
However, these benchmarks are all English-based, making them insufficient to judge the RAG abilities in Korean.
To this end, we have developed an internal FACTs-like Korean benchmark for evaluating RAG abilities, called RAG-General-Bench.
In RAG-General-Bench, human annotators manually constructed the dataset with context, instruction, and reference answer, allowing the evaluation of helpfulness as well. 
% Since reference answer exists, helpfulness can also be evaluated.
% It focued on RAG-specific tasks similar with FACTs.
% In \autoref{rag-ko-eval-data}, benchmark consists of a total of 115 samples, categorized into 27 subcategories, providing a diverse set of scenarios for evaluation. There are 4 samples of each category in \autoref{appendix:rag-bench-example}.
The benchmark consists of a total of 115 samples, categorized into 27 subcategories, providing a diverse set of scenarios for evaluation. There are 4 samples of each category in \autoref{appendix:rag-bench-example}.

% The evaluation of diverse models of korean RAG scenarios is presented in \autoref{fig:rag-main-performance}.
% After our training process, Kanana Essence 9.8B RAG achieved helpfulness while maintaining 91.4\% of GPT-4o's grounding performance. So we comfirmed that Kanana model can sufficiently achieve grounding performance against oracle model.

% The evaluation of diverse models of korean RAG scenarios is presented in \autoref{fig:rag-main-performance}.
% After our training process, Phase 2 model outperformed GPT-4o in grounding performance but its helpfulness fell short of both the base model and other open models.
% Meanwhile, Phase 3 improved helpfulness while maintaining 91.4\% of GPT-4o's grounding performance. So we comfirmed that Kanana model can sufficiently achieve grounding performance against oracle model.

    % We train Kanana Essence model following training process in \autoref{fig:model-recipe}.
    % We conduct ablations while fixing SFT-DPO flow and model merge is utilized after DPO to maintain helpfulness and instruction-following performance.

    % In phase1, we use 2.1M unique samples for training, including SynQA-SFT Collection.
    % To maintain the general capabilities of the base model, around 40\% of the total samples were replayed using Kanana-SFT dataset.
    % Sequence packing was employed to ensure contamination-free training, allowing the attention mechanism to function solely within individual samples.
    % We set maximum learning rate to $5\times10^{-6}$, the warmup steps to 200, minimum learning rate to 10\% of peak lr and trained with 3 epochs.
    % In phase2, We further train supervised fine-tuned model using 250K unique samples from SynQA-DPO Collection.
    % We set the maximum learning rate to $1\times10^{-7}$, the warmup steps to 200, and the minimum learning rate to 0.1 and trained with 3 epochs. In phase3, we merged Kanana-Inst and DPO model in a 1:1 ratio.
    % It enables an ensemble effect without increasing inference time \citep{wortsman2022modelsoupsaveragingweights}. 
    
  
    
% \begin{figure}[h]
%     \centering
%     \resizebox{0.8\textwidth}{!}{%
%         \includegraphics[width=\textwidth]{figures/rag/model-recipe.pdf}
%     }
%     \caption{Training Process}
%     \label{fig:model-recipe}
% \end{figure}

==> colm2025_legacy.tex <==
% colm2025 document legacy
\section{Submission of conference papers to COLM 2025}

COLM requires electronic submissions, processed by
\url{https://openreview.net/}. See COLM's website for more instructions.
The format for the submissions is a variant of the NeurIPS and ICLR formats.
Please read carefully the instructions below, and follow them
faithfully.


\subsection{Style}

Papers to be submitted to COLM 2025 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the COLM \LaTeX{} style files obtainable at the
COLM website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsubsection{Copy Options}

If your paper is ultimately accepted, the option {\tt
  {\textbackslash}final} should be set  for the {\tt {\textbackslash}usepackage[submission]\{colm2025\_conference\}} command for the camera ready version. The {\tt submission} options is the default, and is to be used for all submissions during the review process. It also turns on the line numbers. If you wish to submit a preprint, the option {\tt preprint} should be used.
  
  

\subsection{Retrieval of style files}

The style files for COLM and other conference information are available online at:
\begin{center}
   \url{http://www.colmweb.org/}
\end{center}
The file \verb+colm2025_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your COLM paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+colm2025_conference.sty+ and \verb+colm2025_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+colm2025_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Palatino is the
preferred typeface throughout, and is mandatory for the main text. Paragraphs are separated by 1/2~line space, with no indentation. 

Paper title is 17~point and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Please verify that any custom header information you may add does not override the style defined in this document. This has been known to occur especially when submissions are converted to a new template from a previous one (i.e., for re-submission to a different venue). 

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgements, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

We strongly recommend following arXiv's guidelines for making your paper friendly for HTML conversion: \url{https://info.arxiv.org/help/submit_latex_best_practices.html}.


\section{Headings: first level}
\label{headings}

First level headings are in lower case (except for first word and proper nouns), bold face,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in lower case (except for first word and proper nouns), bold face,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in lower case (except for first word and proper nouns), bold face, italics, 
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Vaswani+2017} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Transformers are a key tool
for developing language models~\citep{Vaswani+2017}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. Any text within the figure must be readable. We ask to not use font sizes below {\tt small}. We strongly recommend to use vector representations (e.g., pdf or svg) for all diagrams. 
We strongly recommend positioning all figures at the top or bottom of the page.

The figure number and caption always appear below the figure. Place one line space before the figure caption, and one line space after the figure. The figure caption is lower case (except for first word and proper nouns); figures are numbered consecutively.
Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[t]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn tables. The table number and title always appear below the table. See Table~\ref{sample-table}. Please do not use font sizes below {\tt small} in tables. We recommend using {\tt booktabs} or a similar package to style tables. 
We strongly recommend positioning all tables at the top or bottom of the page.

Place one line space before the table title, one line space after the table title, and one line space after the table. The table title must be lowercase (except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\begin{center}
\begin{tabular}{ll}
\toprule
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION} \\
\midrule
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\bottomrule
\end{tabular}
\end{center}
\caption{Sample table title}\label{sample-table}
\end{table}




\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

